A 9-Month Hubble Space Telescope Near-UV Survey of M87. I. Light and Color Curves of 94 Novae, and a Re-determination of the Nova Rate

M87 has been monitored with a cadence of 5 days over a 9 month-long span through the near-ultraviolet (NUV:F275W) and optical (F606W) filters of the Wide Field Camera 3 (WFC3) of the $\textit{Hubble Space Telescope}$. This unprecedented dataset yields the NUV and optical light and color curves of 94 M87 novae, characterizing the outburst and decline properties of the largest extragalactic nova dataset in the literature (after M31 and M81). We test and confirm nova modelers' prediction that recurrent novae cannot erupt more frequently that once every 45 days; show that there are zero rapidly recurring novae in the central $\sim$ 1/3 of M87 with recurrence times $ < $ 130 days; demonstrate that novae closely follow the K-band light of M87 to within a few arcsec of the galaxy nucleus; show that nova NUV light curves are as heterogeneous as their optical counterparts, and usually peak 5 to 30 days after visible light maximum; determine our observations' annual detection completeness to be 71 - 77\%; and measure the rate Rnova of nova eruptions in M87 as $352_{-37}^{+37}$/yr. The corresponding luminosity-specific classical nova rate for this galaxy is $7.91_{-1.20}^{+1.20}/yr/10^{10}L_\odot,_{K}$. These rates confirm that ground-based observations of extragalactic novae miss most faint, fast novae and those near the centers of galaxies. An annual M87 nova rate of 300 or more seems inescapable. A luminosity-specific nova rate of $\sim$ $7 - 10/yr/10^{10}L_\odot,_{K}$ in ${\it all}$ types of galaxies is indicated by the data available in 2023.

==> package/tables/shortened_big_phot_paper_table.tex <==
\startlongtable
\begin{deluxetable}{lccccccccc}
\tablewidth{0pt}
\tabletypesize{\footnotesize}
\tablecolumns{9}
\tablecaption{M87 Nova Lightcurve Data}
\tablecomments{\textbf{Table \ref{tab:big_phot} is published in its entirety, with full data for all 53 epochs for all 94 novae, in the machine-readable format. A portion is shown here for guidance regarding its form and content. The precise time of the ``First Ep" is MJD 57705.0605.}}
\tablehead{ \colhead{Epoch} & \colhead{Days since} & \colhead{Days since} &\colhead{Days since} &  \colhead{$V$} & \colhead{$V_{err}$} & \colhead{$U$} & \colhead{$U_{err}$} & \colhead{$(U-V)$} & \colhead{$(U-V)_{err}$} \\ \# & First Ep & F606W Peak & F275W Peak & mag & mag & mag & mag & mag & mag}
\startdata
\multicolumn{10}{c}{M87 Nova 1} \\
\hline\\
44 & 215.26 & -19.87 & -19.87 & $>25.23$ & $\cdots$ & $>25.05$ & $\cdots$ & $\cdots$ & $\cdots$ \\
45 & 220.48 & -14.65 & -14.65 & $>25.31$ & $\cdots$ & $>25.02$ & $\cdots$ & $\cdots$ & $\cdots$ \\
46 & 225.58 & -9.55 & -9.55 & $25.30$ & $0.53$ & $23.96$ & $0.21$ & $-1.34$ & $0.57$ \\
47 & 230.23 & -4.90 & -4.90 & $23.89$ & $0.15$ & $>24.43$ & $\cdots$ & $\cdots$ & $\cdots$ \\
48 & 235.13 & 0.00 & 0.00 & $21.56$ & $0.02$ & $20.72$ & $0.02$ & $-0.85$ & $0.03$ \\
49 & 240.66 & 5.55 & 5.51 & $22.65$ & $0.05$ & $23.48$ & $0.14$ & $0.82$ & $0.15$ \\
50 & 245.26 & 10.13 & 10.13 & $23.13$ & $0.08$ & $23.28$ & $0.13$ & $0.15$ & $0.15$ \\
51 & 250.36 & 15.23 & 15.23 & $23.94$ & $0.16$ & $23.35$ & $0.13$ & $-0.60$ & $0.21$ \\
52 & 255.39 & 20.26 & 20.26 & $24.66$ & $0.30$ & $24.22$ & $0.29$ & $-0.44$ & $0.42$ \\
53 & 260.29 & 25.17 & 25.17 & $25.50$ & $0.65$ & $25.09$ & $0.58$ & $-0.41$ & $0.87$ \\
\hline
\multicolumn{10}{c}{M87 Nova 2} \\
\hline\\
1 & 0.00 & -5.03 & 0.00 & $22.56$ & $0.02$ & $21.87$ & $0.05$ & $-0.69$ & $0.05$ \\
2 & 5.03 & 0.00 & 5.03 & $22.08$ & $0.01$ & $23.94$ & $0.22$ & $1.86$ & $0.22$ \\
3 & 10.93 & 5.90 & 10.93 & $22.86$ & $0.02$ & $23.05$ & $0.10$ & $0.19$ & $0.10$ \\
4 & 15.04 & 10.00 & 15.04 & $23.90$ & $0.06$ & $23.32$ & $0.12$ & $-0.59$ & $0.13$ \\
5 & 20.17 & 15.16 & 20.15 & $24.08$ & $0.07$ & $23.37$ & $0.13$ & $-0.71$ & $0.14$ \\
6 & 25.90 & 20.87 & 25.90 & $25.12$ & $0.16$ & $24.37$ & $0.28$ & $-0.75$ & $0.32$ \\
7 & 30.54 & 25.50 & 30.54 & $26.69$ & $0.63$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ \\
8 & 35.77 & 30.73 & 35.77 & $>26.45$ & $\cdots$ & $>25.16$ & $\cdots$ & $\cdots$ & $\cdots$ \\
9 & 40.01 & 34.97 & 40.01 & $>26.40$ & $\cdots$ & $>25.20$ & $\cdots$ & $\cdots$ & $\cdots$ \\
\hline
\multicolumn{10}{c}{M87 Nova 3} \\
\hline\\
4 & 15.04 & -10.86 & -10.86 & $>27.05$ & $\cdots$ & $>25.10$ & $\cdots$ & $\cdots$ & $\cdots$ \\
5 & 20.17 & -5.71 & -5.75 & $>27.08$ & $\cdots$ & $>25.18$ & $\cdots$ & $\cdots$ & $\cdots$ \\
6 & 25.90 & 0.00 & 0.00 & $22.27$ & $0.01$ & $22.25$ & $0.05$ & $-0.02$ & $0.06$ \\
7 & 30.54 & 4.64 & 4.64 & $24.18$ & $0.04$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ \\
8 & 35.77 & 9.87 & 9.87 & $24.75$ & $0.07$ & $22.86$ & $0.08$ & $-1.89$ & $0.11$ \\
9 & 40.01 & 14.11 & 14.11 & $25.12$ & $0.10$ & $23.07$ & $0.10$ & $-2.04$ & $0.14$ \\
10 & 45.04 & 19.14 & 19.14 & $25.38$ & $0.12$ & $23.46$ & $0.13$ & $-1.92$ & $0.17$ \\
11 & 50.01 & 24.11 & 24.11 & $25.95$ & $0.20$ & $23.85$ & $0.18$ & $-2.10$ & $0.27$ \\
12 & 55.17 & 29.27 & 29.27 & $26.00$ & $0.21$ & $23.76$ & $0.17$ & $-2.24$ & $0.27$ \\
13 & 60.07 & 34.17 & 34.17 & $26.21$ & $0.25$ & $24.24$ & $0.23$ & $-1.97$ & $0.34$ \\
14 & 65.13 & 39.25 & 39.21 & $26.55$ & $0.34$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ \\
15 & 70.05 & 44.17 & 44.12 & $26.57$ & $0.34$ & $>24.63$ & $\cdots$ & $\cdots$ & $\cdots$ \\
16 & 75.58 & 49.68 & 49.68 & $26.37$ & $0.27$ & $>24.35$ & $\cdots$ & $\cdots$ & $\cdots$ \\
17 & 80.54 & 54.64 & 54.64 & $>26.87$ & $\cdots$ & $>25.21$ & $\cdots$ & $\cdots$ & $\cdots$ \\
18 & 85.51 & 59.61 & 59.61 & $>27.14$ & $\cdots$ & $>24.95$ & $\cdots$ & $\cdots$ & $\cdots$ \\
\hline
\multicolumn{10}{c}{M87 Nova 4} \\
\hline\\
42 & 205.46 & -20.12 & -15.02 & $>27.75$ & $\cdots$ & $>25.26$ & $\cdots$ & $\cdots$ & $\cdots$ \\
43 & 210.49 & -15.09 & -9.99 & $>27.43$ & $\cdots$ & $>25.27$ & $\cdots$ & $\cdots$ & $\cdots$ \\
44 & 215.26 & -10.32 & -5.22 & $25.64$ & $0.09$ & $>25.35$ & $\cdots$ & $\cdots$ & $\cdots$ \\
45 & 220.48 & -5.10 & 0.00 & $22.65$ & $0.01$ & $23.47$ & $0.12$ & $0.82$ & $0.12$ \\
46 & 225.58 & 0.00 & 5.10 & $22.42$ & $0.01$ & $24.63$ & $0.32$ & $2.21$ & $0.32$ \\
47 & 230.23 & 4.65 & 9.75 & $23.01$ & $0.02$ & $24.06$ & $0.19$ & $1.05$ & $0.19$ \\
48 & 235.13 & 9.55 & 14.65 & $23.33$ & $0.02$ & $23.66$ & $0.15$ & $0.33$ & $0.15$ \\
49 & 240.66 & 15.10 & 20.16 & $24.18$ & $0.03$ & $24.51$ & $0.31$ & $0.32$ & $0.31$ \\
50 & 245.26 & 19.68 & 24.78 & $24.95$ & $0.06$ & $24.52$ & $0.29$ & $-0.43$ & $0.29$ \\
51 & 250.36 & 24.78 & 29.88 & $25.86$ & $0.12$ & $>25.13$ & $\cdots$ & $\cdots$ & $\cdots$ \\
52 & 255.39 & 29.81 & 34.91 & $27.47$ & $0.49$ & $>25.26$ & $\cdots$ & $\cdots$ & $\cdots$ \\
53 & 260.29 & 34.71 & 39.81 & $>27.39$ & $\cdots$ & $>25.31$ & $\cdots$ & $\cdots$ & $\cdots$ \\
\hline
\multicolumn{10}{c}{M87 Nova 5} \\
\hline\\
28 & 135.19 & -10.46 & -10.46 & $>25.08$ & $\cdots$ & $>24.93$ & $\cdots$ & $\cdots$ & $\cdots$ \\
29 & 140.48 & -5.17 & -5.17 & $>25.45$ & $\cdots$ & $>24.83$ & $\cdots$ & $\cdots$ & $\cdots$ \\
30 & 145.65 & 0.00 & 0.00 & $22.52$ & $0.04$ & $20.57$ & $0.02$ & $-1.95$ & $0.05$ \\
31 & 150.15 & 4.50 & 4.50 & $24.76$ & $0.29$ & $23.67$ & $0.19$ & $-1.09$ & $0.35$ \\
32 & 155.45 & 9.80 & 9.80 & $>25.39$ & $\cdots$ & $>23.66$ & $\cdots$ & $\cdots$ & $\cdots$ \\
33 & 160.42 & 14.77 & 14.77 & $>25.41$ & $\cdots$ & $>24.72$ & $\cdots$ & $\cdots$ & $\cdots$ \\
\hline
\multicolumn{10}{c}{M87 Nova 6} \\
\hline\\
23 & 110.54 & -10.39 & -10.35 & $>27.70$ & $\cdots$ & $>25.21$ & $\cdots$ & $\cdots$ & $\cdots$ \\
24 & 115.51 & -5.43 & -5.38 & $>27.79$ & $\cdots$ & $>25.15$ & $\cdots$ & $\cdots$ & $\cdots$ \\
25 & 120.91 & 0.00 & 0.00 & $22.66$ & $0.01$ & $22.50$ & $0.07$ & $-0.16$ & $0.07$ \\
26 & 125.65 & 4.71 & 4.76 & $23.89$ & $0.03$ & $22.58$ & $0.07$ & $-1.31$ & $0.08$ \\
27 & 130.35 & 9.41 & 9.46 & $24.67$ & $0.05$ & $22.50$ & $0.07$ & $-2.17$ & $0.08$ \\
28 & 135.19 & 14.25 & 14.30 & $25.45$ & $0.08$ & $23.18$ & $0.10$ & $-2.27$ & $0.13$ \\
29 & 140.48 & 19.55 & 19.59 & $25.93$ & $0.12$ & $23.38$ & $0.12$ & $-2.54$ & $0.16$ \\
30 & 145.65 & 24.71 & 24.76 & $26.19$ & $0.15$ & $23.82$ & $0.17$ & $-2.37$ & $0.23$ \\
31 & 150.15 & 29.22 & 29.26 & $26.01$ & $0.13$ & $23.84$ & $0.16$ & $-2.17$ & $0.20$ \\
32 & 155.45 & 34.51 & 34.56 & $26.57$ & $0.20$ & $23.97$ & $0.17$ & $-2.60$ & $0.26$ \\
33 & 160.42 & 39.48 & 39.53 & $26.25$ & $0.15$ & $24.67$ & $0.32$ & $-1.58$ & $0.35$ \\
34 & 165.65 & 44.71 & 44.76 & $26.22$ & $0.15$ & $24.71$ & $0.32$ & $-1.52$ & $0.35$ \\
35 & 170.35 & 49.41 & 49.46 & $26.38$ & $0.17$ & $24.82$ & $0.36$ & $-1.56$ & $0.40$ \\
36 & 175.24 & 54.30 & 54.35 & $26.72$ & $0.23$ & $25.16$ & $0.50$ & $-1.55$ & $0.55$ \\
37 & 180.49 & 59.55 & 59.60 & $27.05$ & $0.30$ & $24.55$ & $0.29$ & $-2.50$ & $0.41$ \\
38 & 185.39 & 64.45 & 64.50 & $27.04$ & $0.31$ & $25.08$ & $0.46$ & $-1.96$ & $0.56$ \\
39 & 190.36 & 69.42 & 69.47 & $>26.72$ & $\cdots$ & $>25.13$ & $\cdots$ & $\cdots$ & $\cdots$ \\
40 & 195.12 & 74.19 & 74.23 & $>26.54$ & $\cdots$ & $25.04$ & $0.42$ & $\cdots$ & $\cdots$ \\
41 & 200.69 & 79.75 & 79.80 & $>27.14$ & $\cdots$ & $>24.99$ & $\cdots$ & $\cdots$ & $\cdots$ \\
42 & 205.46 & 84.52 & 84.56 & $>26.56$ & $\cdots$ & $>24.89$ & $\cdots$ & $\cdots$ & $\cdots$ \\
\hline
\multicolumn{10}{c}{M87 Nova 7} \\
\hline\\
0 & 260.29 & 260.29 & 260.29 & $>23.67$ & $\cdots$ & $>23.17$ & $\cdots$ & $\cdots$ & $\cdots$ \\
1 & 0.00 & 0.00 & 0.00 & $22.68$ & $0.05$ & $21.79$ & $0.04$ & $-0.89$ & $0.07$ \\
2 & 5.03 & 5.03 & 5.03 & $>23.76$ & $\cdots$ & $>23.71$ & $\cdots$ & $\cdots$ & $\cdots$ \\
3 & 10.93 & 10.93 & 10.93 & $>23.55$ & $\cdots$ & $>23.36$ & $\cdots$ & $\cdots$ & $\cdots$ \\
\hline
\multicolumn{10}{c}{M87 Nova 8} \\
\hline\\
43 & 210.49 & -9.99 & -15.09 & $>24.98$ & $\cdots$ & $>24.92$ & $\cdots$ & $\cdots$ & $\cdots$ \\
44 & 215.26 & -5.22 & -10.32 & $>25.01$ & $\cdots$ & $>24.82$ & $\cdots$ & $\cdots$ & $\cdots$ \\
45 & 220.48 & 0.00 & -5.10 & $22.86$ & $0.08$ & $22.96$ & $0.10$ & $0.09$ & $0.12$ \\
46 & 225.58 & 5.10 & 0.00 & $24.08$ & $0.24$ & $22.92$ & $0.09$ & $-1.15$ & $0.25$ \\
47 & 230.23 & 9.75 & 4.65 & $24.68$ & $0.42$ & $23.38$ & $0.14$ & $-1.30$ & $0.44$ \\
48 & 235.13 & 14.65 & 9.55 & $>24.95$ & $\cdots$ & $23.60$ & $0.16$ & $\cdots$ & $\cdots$ \\
49 & 240.66 & 20.20 & 15.06 & $>24.65$ & $\cdots$ & $24.19$ & $0.27$ & $\cdots$ & $\cdots$ \\
50 & 245.26 & 24.78 & 19.68 & $>25.00$ & $\cdots$ & $23.78$ & $0.20$ & $\cdots$ & $\cdots$ \\
51 & 250.36 & 29.88 & 24.78 & $>25.03$ & $\cdots$ & $>24.35$ & $\cdots$ & $\cdots$ & $\cdots$ \\
52 & 255.39 & 34.91 & 29.81 & $>24.90$ & $\cdots$ & $>24.34$ & $\cdots$ & $\cdots$ & $\cdots$ \\
\hline
\multicolumn{10}{c}{M87 Nova 9} \\
\hline\\
44 & 215.26 & -10.32 & -10.32 & $>27.49$ & $\cdots$ & $>25.25$ & $\cdots$ & $\cdots$ & $\cdots$ \\
45 & 220.48 & -5.10 & -5.10 & $>27.82$ & $\cdots$ & $>25.31$ & $\cdots$ & $\cdots$ & $\cdots$ \\
46 & 225.58 & 0.00 & 0.00 & $23.08$ & $0.02$ & $21.65$ & $0.03$ & $-1.43$ & $0.04$ \\
47 & 230.23 & 4.65 & 4.65 & $23.75$ & $0.02$ & $24.38$ & $0.26$ & $0.63$ & $0.26$ \\
48 & 235.13 & 9.55 & 9.55 & $24.55$ & $0.04$ & $23.60$ & $0.14$ & $-0.95$ & $0.15$ \\
49 & 240.66 & 15.10 & 15.06 & $24.86$ & $0.05$ & $23.58$ & $0.14$ & $-1.28$ & $0.15$ \\
50 & 245.26 & 19.68 & 19.68 & $25.25$ & $0.06$ & $23.72$ & $0.14$ & $-1.53$ & $0.16$ \\
51 & 250.36 & 24.78 & 24.78 & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ \\
52 & 255.39 & 29.81 & 29.81 & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ \\
\hline
\multicolumn{10}{c}{M87 Nova 10} \\
\hline\\
19 & 90.61 & -35.04 & -49.87 & $>25.95$ & $\cdots$ & $>24.46$ & $\cdots$ & $\cdots$ & $\cdots$ \\
20 & 95.31 & -30.34 & -45.17 & $>26.38$ & $\cdots$ & $>25.09$ & $\cdots$ & $\cdots$ & $\cdots$ \\
21 & 100.50 & -25.13 & -40.00 & $26.50$ & $0.59$ & $>25.19$ & $\cdots$ & $\cdots$ & $\cdots$ \\
22 & 105.23 & -20.42 & -35.25 & $>25.84$ & $\cdots$ & $>25.07$ & $\cdots$ & $\cdots$ & $\cdots$ \\
23 & 110.54 & -15.10 & -29.94 & $>26.18$ & $\cdots$ & $>25.18$ & $\cdots$ & $\cdots$ & $\cdots$ \\
24 & 115.51 & -10.14 & -24.97 & $>26.38$ & $\cdots$ & $>25.14$ & $\cdots$ & $\cdots$ & $\cdots$ \\
25 & 120.91 & -4.71 & -19.59 & $26.41$ & $0.56$ & $>25.03$ & $\cdots$ & $\cdots$ & $\cdots$ \\
26 & 125.65 & 0.00 & -14.84 & $23.10$ & $0.03$ & $23.66$ & $0.18$ & $0.56$ & $0.18$ \\
27 & 130.35 & 4.70 & -10.13 & $\cdots$ & $\cdots$ & $24.06$ & $0.27$ & $\cdots$ & $\cdots$ \\
28 & 135.19 & 9.54 & -5.30 & $25.14$ & $0.17$ & $23.31$ & $0.14$ & $-1.82$ & $0.22$ \\
29 & 140.48 & 14.84 & 0.00 & $25.63$ & $0.26$ & $23.28$ & $0.13$ & $-2.35$ & $0.29$ \\
30 & 145.65 & 20.00 & 5.17 & $25.56$ & $0.25$ & $23.42$ & $0.14$ & $-2.14$ & $0.29$ \\
31 & 150.15 & 24.51 & 9.67 & $26.10$ & $0.40$ & $23.73$ & $0.19$ & $-2.36$ & $0.44$ \\
32 & 155.45 & 29.80 & 14.97 & $25.98$ & $0.36$ & $24.43$ & $0.31$ & $-1.55$ & $0.48$ \\
33 & 160.42 & 34.77 & 19.94 & $26.57$ & $0.64$ & $>24.79$ & $\cdots$ & $\cdots$ & $\cdots$ \\
34 & 165.65 & 40.00 & 25.17 & $26.16$ & $0.43$ & $24.62$ & $0.38$ & $-1.54$ & $0.58$ \\
35 & 170.35 & 44.71 & 29.87 & $>26.32$ & $\cdots$ & $>24.86$ & $\cdots$ & $\cdots$ & $\cdots$ \\
36 & 175.24 & 49.59 & 34.75 & $26.32$ & $0.50$ & $>24.30$ & $\cdots$ & $\cdots$ & $\cdots$ \\
37 & 180.49 & 54.84 & 40.00 & $>26.26$ & $\cdots$ & $24.58$ & $0.36$ & $\cdots$ & $\cdots$ \\
38 & 185.39 & 59.74 & 44.91 & $26.47$ & $0.58$ & $>24.33$ & $\cdots$ & $\cdots$ & $\cdots$ \\
39 & 190.36 & 64.71 & 49.87 & $>26.16$ & $\cdots$ & $>24.25$ & $\cdots$ & $\cdots$ & $\cdots$ \\
40 & 195.12 & 69.48 & 54.64 & $>26.44$ & $\cdots$ & $>25.10$ & $\cdots$ & $\cdots$ & $\cdots$ \\
41 & 200.69 & 75.04 & 60.20 & $26.22$ & $0.45$ & $>25.07$ & $\cdots$ & $\cdots$ & $\cdots$ \\
42 & 205.46 & 79.81 & 64.97 & $26.41$ & $0.55$ & $>25.08$ & $\cdots$ & $\cdots$ & $\cdots$ \\
43 & 210.49 & 84.84 & 70.00 & $26.35$ & $0.49$ & $>24.61$ & $\cdots$ & $\cdots$ & $\cdots$ \\
44 & 215.26 & 89.61 & 74.77 & $>26.38$ & $\cdots$ & $>25.03$ & $\cdots$ & $\cdots$ & $\cdots$ \\
45 & 220.48 & 94.83 & 80.00 & $>26.43$ & $\cdots$ & $>25.10$ & $\cdots$ & $\cdots$ & $\cdots$ \\
46 & 225.58 & 99.93 & 85.10 & $>26.36$ & $\cdots$ & $>24.56$ & $\cdots$ & $\cdots$ & $\cdots$ \\
47 & 230.23 & 104.58 & 89.74 & $>26.33$ & $\cdots$ & $>25.11$ & $\cdots$ & $\cdots$ & $\cdots$ \\
48 & 235.13 & 109.48 & 94.64 & $26.65$ & $0.70$ & $>25.03$ & $\cdots$ & $\cdots$ & $\cdots$ \\
49 & 240.66 & 115.03 & 100.15 & $26.58$ & $0.64$ & $>24.31$ & $\cdots$ & $\cdots$ & $\cdots$ \\
50 & 245.26 & 119.61 & 104.78 & $>26.28$ & $\cdots$ & $>25.13$ & $\cdots$ & $\cdots$ & $\cdots$ \\
51 & 250.36 & 124.71 & 109.87 & $>26.41$ & $\cdots$ & $>25.16$ & $\cdots$ & $\cdots$ & $\cdots$ \\
52 & 255.39 & 129.74 & 114.91 & $26.28$ & $0.48$ & $>24.41$ & $\cdots$ & $\cdots$ & $\cdots$ \\
53 & 260.29 & 134.64 & 119.81 & $>26.33$ & $\cdots$ & $>25.05$ & $\cdots$ & $\cdots$ & $\cdots$ \\
\hline
\multicolumn{10}{c}{M87 Nova 11} \\
\hline\\
3 & 10.93 & -9.26 & -14.97 & $>26.06$ & $\cdots$ & $>25.12$ & $\cdots$ & $\cdots$ & $\cdots$ \\
4 & 15.04 & -5.16 & -10.86 & $>25.96$ & $\cdots$ & $>24.57$ & $\cdots$ & $\cdots$ & $\cdots$ \\
5 & 20.17 & 0.00 & -5.75 & $23.12$ & $0.04$ & $23.63$ & $0.17$ & $0.51$ & $0.17$ \\
6 & 25.90 & 5.71 & 0.00 & $24.86$ & $0.19$ & $22.73$ & $0.08$ & $-2.13$ & $0.21$ \\
7 & 30.54 & 10.34 & 4.64 & $>25.42$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ \\
8 & 35.77 & 15.57 & 9.87 & $>26.03$ & $\cdots$ & $24.14$ & $0.24$ & $\cdots$ & $\cdots$ \\
9 & 40.01 & 19.81 & 14.11 & $>25.35$ & $\cdots$ & $>24.47$ & $\cdots$ & $\cdots$ & $\cdots$ \\
10 & 45.04 & 24.85 & 19.14 & $>25.45$ & $\cdots$ & $>24.06$ & $\cdots$ & $\cdots$ & $\cdots$ \\
\hline
\multicolumn{10}{c}{M87 Nova 12} \\
\hline\\
3 & 10.93 & -9.26 & -9.22 & $>27.02$ & $\cdots$ & $>24.62$ & $\cdots$ & $\cdots$ & $\cdots$ \\
4 & 15.04 & -5.16 & -5.11 & $>26.97$ & $\cdots$ & $>25.21$ & $\cdots$ & $\cdots$ & $\cdots$ \\
5 & 20.17 & 0.00 & 0.00 & $23.13$ & $0.02$ & $21.49$ & $0.03$ & $-1.64$ & $0.04$ \\
6 & 25.90 & 5.71 & 5.75 & $24.56$ & $0.06$ & $22.70$ & $0.07$ & $-1.86$ & $0.09$ \\
7 & 30.54 & 10.34 & 10.39 & $25.66$ & $0.15$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ \\
8 & 35.77 & 15.57 & 15.62 & $26.07$ & $0.21$ & $23.58$ & $0.15$ & $-2.49$ & $0.26$ \\
9 & 40.01 & 19.81 & 19.86 & $26.49$ & $0.32$ & $24.06$ & $0.22$ & $-2.43$ & $0.39$ \\
10 & 45.04 & 24.85 & 24.89 & $26.43$ & $0.30$ & $24.33$ & $0.27$ & $-2.10$ & $0.41$ \\
11 & 50.01 & 29.81 & 29.86 & $27.05$ & $0.58$ & $24.74$ & $0.41$ & $-2.31$ & $0.71$ \\
12 & 55.17 & 34.98 & 35.02 & $>26.76$ & $\cdots$ & $>24.65$ & $\cdots$ & $\cdots$ & $\cdots$ \\
13 & 60.07 & 39.88 & 39.92 & $>26.85$ & $\cdots$ & $24.46$ & $0.31$ & $\cdots$ & $\cdots$ \\
14 & 65.13 & 44.95 & 44.96 & $>26.99$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ \\
15 & 70.05 & 49.88 & 49.87 & $>27.03$ & $\cdots$ & $24.77$ & $0.41$ & $\cdots$ & $\cdots$ \\
16 & 75.58 & 55.38 & 55.43 & $>27.03$ & $\cdots$ & $>24.80$ & $\cdots$ & $\cdots$ & $\cdots$ \\
17 & 80.54 & 60.35 & 60.39 & $>27.05$ & $\cdots$ & $>25.11$ & $\cdots$ & $\cdots$ & $\cdots$ \\
18 & 85.51 & 65.32 & 65.36 & $>27.02$ & $\cdots$ & $>25.02$ & $\cdots$ & $\cdots$ & $\cdots$ \\
19 & 90.61 & 70.42 & 70.46 & $>27.06$ & $\cdots$ & $>24.60$ & $\cdots$ & $\cdots$ & $\cdots$ \\
20 & 95.31 & 75.12 & 75.16 & $27.13$ & $0.58$ & $>24.82$ & $\cdots$ & $\cdots$ & $\cdots$ \\
21 & 100.50 & 80.32 & 80.33 & $>27.10$ & $\cdots$ & $>25.23$ & $\cdots$ & $\cdots$ & $\cdots$ \\
22 & 105.23 & 85.04 & 85.08 & $>27.02$ & $\cdots$ & $>25.06$ & $\cdots$ & $\cdots$ & $\cdots$ \\
\hline
\multicolumn{10}{c}{M87 Nova 13} \\
\hline\\
41 & 200.69 & -9.80 & -24.89 & $>26.78$ & $\cdots$ & $>25.01$ & $\cdots$ & $\cdots$ & $\cdots$ \\
42 & 205.46 & -5.03 & -20.12 & $>26.78$ & $\cdots$ & $>25.13$ & $\cdots$ & $\cdots$ & $\cdots$ \\
43 & 210.49 & 0.00 & -15.09 & $23.23$ & $0.03$ & $>24.87$ & $\cdots$ & $\cdots$ & $\cdots$ \\
44 & 215.26 & 4.77 & -10.32 & $24.37$ & $0.06$ & $23.42$ & $0.14$ & $-0.95$ & $0.15$ \\
45 & 220.48 & 9.99 & -5.10 & $24.89$ & $0.10$ & $23.39$ & $0.13$ & $-1.49$ & $0.16$ \\
46 & 225.58 & 15.09 & 0.00 & $25.76$ & $0.22$ & $23.21$ & $0.11$ & $-2.56$ & $0.25$ \\
47 & 230.23 & 19.74 & 4.65 & $26.06$ & $0.28$ & $23.89$ & $0.21$ & $-2.17$ & $0.35$ \\
48 & 235.13 & 24.64 & 9.55 & $26.35$ & $0.39$ & $23.75$ & $0.19$ & $-2.60$ & $0.44$ \\
49 & 240.66 & 30.19 & 15.06 & $26.30$ & $0.35$ & $23.98$ & $0.21$ & $-2.32$ & $0.41$ \\
50 & 245.26 & 34.77 & 19.68 & $>26.58$ & $\cdots$ & $>25.12$ & $\cdots$ & $\cdots$ & $\cdots$ \\
51 & 250.36 & 39.87 & 24.78 & $26.39$ & $0.40$ & $24.19$ & $0.28$ & $-2.20$ & $0.49$ \\
52 & 255.39 & 44.90 & 29.81 & $>26.77$ & $\cdots$ & $>24.64$ & $\cdots$ & $\cdots$ & $\cdots$ \\
53 & 260.29 & 49.80 & 34.71 & $>26.77$ & $\cdots$ & $>24.49$ & $\cdots$ & $\cdots$ & $\cdots$ \\
\hline
\multicolumn{10}{c}{M87 Nova 14} \\
\hline\\
4 & 15.04 & -30.00 & -34.97 & $>27.29$ & $\cdots$ & $>25.25$ & $\cdots$ & $\cdots$ & $\cdots$ \\
5 & 20.17 & -24.85 & -29.86 & $>27.30$ & $\cdots$ & $>25.12$ & $\cdots$ & $\cdots$ & $\cdots$ \\
6 & 25.90 & -19.14 & -24.11 & $>27.22$ & $\cdots$ & $25.37$ & $0.63$ & $\cdots$ & $\cdots$ \\
7 & 30.54 & -14.51 & -19.47 & $>26.88$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ \\
8 & 35.77 & -9.27 & -14.24 & $>26.95$ & $\cdots$ & $>25.15$ & $\cdots$ & $\cdots$ & $\cdots$ \\
9 & 40.01 & -5.03 & -10.00 & $>27.37$ & $\cdots$ & $>25.21$ & $\cdots$ & $\cdots$ & $\cdots$ \\
10 & 45.04 & 0.00 & -4.97 & $23.32$ & $0.02$ & $23.66$ & $0.15$ & $0.33$ & $0.15$ \\
11 & 50.01 & 4.97 & 0.00 & $24.43$ & $0.05$ & $22.93$ & $0.09$ & $-1.49$ & $0.10$ \\
12 & 55.17 & 10.13 & 5.17 & $25.03$ & $0.07$ & $23.27$ & $0.11$ & $-1.75$ & $0.13$ \\
13 & 60.07 & 15.03 & 10.07 & $25.72$ & $0.13$ & $23.37$ & $0.12$ & $-2.35$ & $0.18$ \\
14 & 65.13 & 20.10 & 15.10 & $26.20$ & $0.19$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ \\
15 & 70.05 & 25.03 & 20.02 & $26.60$ & $0.26$ & $24.12$ & $0.21$ & $-2.48$ & $0.34$ \\
16 & 75.58 & 30.54 & 25.57 & $26.32$ & $0.22$ & $24.31$ & $0.25$ & $-2.01$ & $0.33$ \\
17 & 80.54 & 35.50 & 30.54 & $26.72$ & $0.30$ & $24.57$ & $0.32$ & $-2.15$ & $0.44$ \\
18 & 85.51 & 40.47 & 35.50 & $26.82$ & $0.34$ & $>25.07$ & $\cdots$ & $\cdots$ & $\cdots$ \\
19 & 90.61 & 45.57 & 40.60 & $27.01$ & $0.43$ & $>23.96$ & $\cdots$ & $\cdots$ & $\cdots$ \\
20 & 95.31 & 50.27 & 45.30 & $26.86$ & $0.35$ & $>25.19$ & $\cdots$ & $\cdots$ & $\cdots$ \\
21 & 100.50 & 55.47 & 50.47 & $>27.37$ & $\cdots$ & $>24.91$ & $\cdots$ & $\cdots$ & $\cdots$ \\
22 & 105.23 & 60.19 & 55.22 & $\cdots$ & $\cdots$ & $>25.18$ & $\cdots$ & $\cdots$ & $\cdots$ \\
\hline
\multicolumn{10}{c}{M87 Nova 15} \\
\hline\\
27 & 130.35 & -19.80 & -25.10 & $\cdots$ & $\cdots$ & $>24.92$ & $\cdots$ & $\cdots$ & $\cdots$ \\
28 & 135.19 & -14.97 & -20.27 & $\cdots$ & $\cdots$ & $>24.86$ & $\cdots$ & $\cdots$ & $\cdots$ \\
29 & 140.48 & -9.67 & -14.97 & $\cdots$ & $\cdots$ & $24.19$ & $0.31$ & $\cdots$ & $\cdots$ \\
30 & 145.65 & -4.50 & -9.80 & $23.55$ & $0.07$ & $>24.39$ & $\cdots$ & $\cdots$ & $\cdots$ \\
31 & 150.15 & 0.00 & -5.30 & $23.41$ & $0.06$ & $23.61$ & $0.18$ & $0.20$ & $0.19$ \\
32 & 155.45 & 5.30 & 0.00 & $23.45$ & $0.06$ & $22.73$ & $0.08$ & $-0.72$ & $0.10$ \\
33 & 160.42 & 10.27 & 4.97 & $24.38$ & $0.14$ & $23.40$ & $0.13$ & $-0.98$ & $0.19$ \\
34 & 165.65 & 15.50 & 10.20 & $24.64$ & $0.17$ & $23.20$ & $0.12$ & $-1.43$ & $0.21$ \\
35 & 170.35 & 20.20 & 14.90 & $25.03$ & $0.25$ & $23.25$ & $0.11$ & $-1.77$ & $0.28$ \\
36 & 175.24 & 25.09 & 19.79 & $26.15$ & $0.68$ & $>24.13$ & $\cdots$ & $\cdots$ & $\cdots$ \\
37 & 180.49 & 30.33 & 25.04 & $>25.85$ & $\cdots$ & $>23.96$ & $\cdots$ & $\cdots$ & $\cdots$ \\
38 & 185.39 & 35.24 & 29.94 & $>25.93$ & $\cdots$ & $>25.11$ & $\cdots$ & $\cdots$ & $\cdots$ \\
\hline
\multicolumn{10}{c}{M87 Nova 16} \\
\hline\\
21 & 100.50 & -10.03 & -10.06 & $>25.90$ & $\cdots$ & $>24.84$ & $\cdots$ & $\cdots$ & $\cdots$ \\
22 & 105.23 & -5.31 & -5.31 & $>25.96$ & $\cdots$ & $>24.71$ & $\cdots$ & $\cdots$ & $\cdots$ \\
23 & 110.54 & 0.00 & 0.00 & $23.41$ & $0.06$ & $22.86$ & $0.10$ & $-0.55$ & $0.12$ \\
24 & 115.51 & 4.97 & 4.97 & $24.23$ & $0.13$ & $23.01$ & $0.09$ & $-1.22$ & $0.16$ \\
25 & 120.91 & 10.39 & 10.35 & $25.22$ & $0.25$ & $23.31$ & $0.13$ & $-1.91$ & $0.29$ \\
26 & 125.65 & 15.10 & 15.10 & $25.54$ & $0.36$ & $24.48$ & $0.47$ & $-1.06$ & $0.59$ \\
27 & 130.35 & 19.81 & 19.81 & $\cdots$ & $\cdots$ & $>24.11$ & $\cdots$ & $\cdots$ & $\cdots$ \\
28 & 135.19 & 24.64 & 24.64 & $>25.63$ & $\cdots$ & $>23.86$ & $\cdots$ & $\cdots$ & $\cdots$ \\
\hline
\multicolumn{10}{c}{M87 Nova 17} \\
\hline\\
27 & 130.35 & -10.13 & -19.80 & $>26.22$ & $\cdots$ & $>25.03$ & $\cdots$ & $\cdots$ & $\cdots$ \\
28 & 135.19 & -5.30 & -14.97 & $>26.22$ & $\cdots$ & $>24.97$ & $\cdots$ & $\cdots$ & $\cdots$ \\
29 & 140.48 & 0.00 & -9.67 & $23.48$ & $0.05$ & $>24.11$ & $\cdots$ & $\cdots$ & $\cdots$ \\
30 & 145.65 & 5.17 & -4.50 & $24.29$ & $0.09$ & $24.09$ & $0.27$ & $-0.20$ & $0.28$ \\
31 & 150.15 & 9.67 & 0.00 & $24.74$ & $0.14$ & $23.54$ & $0.15$ & $-1.20$ & $0.21$ \\
32 & 155.45 & 14.97 & 5.30 & $25.69$ & $0.33$ & $23.85$ & $0.20$ & $-1.84$ & $0.38$ \\
33 & 160.42 & 19.94 & 10.27 & $25.99$ & $0.43$ & $23.56$ & $0.16$ & $-2.43$ & $0.46$ \\
34 & 165.65 & 25.17 & 15.50 & $>26.06$ & $\cdots$ & $23.87$ & $0.21$ & $\cdots$ & $\cdots$ \\
35 & 170.35 & 29.87 & 20.20 & $>25.74$ & $\cdots$ & $23.60$ & $0.16$ & $\cdots$ & $\cdots$ \\
36 & 175.24 & 34.76 & 25.09 & $>25.87$ & $\cdots$ & $>23.57$ & $\cdots$ & $\cdots$ & $\cdots$ \\
37 & 180.49 & 40.00 & 30.33 & $>26.26$ & $\cdots$ & $>24.60$ & $\cdots$ & $\cdots$ & $\cdots$ \\
\hline
\multicolumn{10}{c}{M87 Nova 18} \\
\hline\\
26 & 125.65 & -9.54 & -20.00 & $>25.28$ & $\cdots$ & $>24.91$ & $\cdots$ & $\cdots$ & $\cdots$ \\
27 & 130.35 & -4.83 & -15.30 & $>25.26$ & $\cdots$ & $>25.04$ & $\cdots$ & $\cdots$ & $\cdots$ \\
28 & 135.19 & 0.00 & -10.46 & $23.56$ & $0.11$ & $>25.01$ & $\cdots$ & $\cdots$ & $\cdots$ \\
29 & 140.48 & 5.30 & -5.17 & $24.43$ & $0.24$ & $23.75$ & $0.19$ & $-0.68$ & $0.31$ \\
30 & 145.65 & 10.46 & 0.00 & $24.89$ & $0.37$ & $23.25$ & $0.13$ & $-1.64$ & $0.39$ \\
31 & 150.15 & 14.97 & 4.50 & $25.39$ & $0.61$ & $23.29$ & $0.14$ & $-2.10$ & $0.62$ \\
32 & 155.45 & 20.27 & 9.80 & $>25.27$ & $\cdots$ & $23.59$ & $0.16$ & $\cdots$ & $\cdots$ \\
33 & 160.42 & 25.23 & 14.77 & $>25.32$ & $\cdots$ & $23.59$ & $0.15$ & $\cdots$ & $\cdots$ \\
34 & 165.65 & 30.46 & 20.00 & $>25.27$ & $\cdots$ & $24.22$ & $0.29$ & $\cdots$ & $\cdots$ \\
35 & 170.35 & 35.17 & 24.70 & $>25.28$ & $\cdots$ & $>25.14$ & $\cdots$ & $\cdots$ & $\cdots$ \\
36 & 175.24 & 40.05 & 29.59 & $>25.26$ & $\cdots$ & $>25.07$ & $\cdots$ & $\cdots$ & $\cdots$ \\
\hline
\multicolumn{10}{c}{M87 Nova 19} \\
\hline\\
38 & 185.39 & -9.73 & -20.07 & $>27.37$ & $\cdots$ & $>25.15$ & $\cdots$ & $\cdots$ & $\cdots$ \\
39 & 190.36 & -4.77 & -15.10 & $>27.46$ & $\cdots$ & $>25.07$ & $\cdots$ & $\cdots$ & $\cdots$ \\
40 & 195.12 & 0.00 & -10.33 & $23.58$ & $0.02$ & $24.33$ & $0.27$ & $0.76$ & $0.28$ \\
41 & 200.69 & 5.56 & -4.77 & $24.19$ & $0.03$ & $23.62$ & $0.16$ & $-0.57$ & $0.17$ \\
42 & 205.46 & 10.33 & 0.00 & $24.68$ & $0.05$ & $23.04$ & $0.10$ & $-1.64$ & $0.11$ \\
43 & 210.49 & 15.36 & 5.03 & $24.80$ & $0.06$ & $23.07$ & $0.10$ & $-1.73$ & $0.11$ \\
44 & 215.26 & 20.13 & 9.80 & $25.65$ & $0.11$ & $23.24$ & $0.11$ & $-2.41$ & $0.16$ \\
45 & 220.48 & 25.36 & 15.02 & $25.65$ & $0.12$ & $23.32$ & $0.12$ & $-2.32$ & $0.17$ \\
46 & 225.58 & 30.45 & 20.12 & $26.08$ & $0.17$ & $23.74$ & $0.17$ & $-2.34$ & $0.23$ \\
47 & 230.23 & 35.10 & 24.77 & $26.13$ & $0.19$ & $23.68$ & $0.16$ & $-2.45$ & $0.25$ \\
48 & 235.13 & 40.00 & 29.67 & $26.96$ & $0.36$ & $24.58$ & $0.35$ & $-2.38$ & $0.50$ \\
49 & 240.66 & 45.56 & 35.18 & $>27.29$ & $\cdots$ & $>25.18$ & $\cdots$ & $\cdots$ & $\cdots$ \\
50 & 245.26 & 50.14 & 39.80 & $>27.28$ & $\cdots$ & $>25.09$ & $\cdots$ & $\cdots$ & $\cdots$ \\
\hline
\multicolumn{10}{c}{M87 Nova 20} \\
\hline\\
15 & 70.05 & -10.47 & -25.29 & $>27.70$ & $\cdots$ & $>25.13$ & $\cdots$ & $\cdots$ & $\cdots$ \\
16 & 75.58 & -4.97 & -19.74 & $>27.71$ & $\cdots$ & $>25.08$ & $\cdots$ & $\cdots$ & $\cdots$ \\
17 & 80.54 & 0.00 & -14.77 & $23.58$ & $0.02$ & $>25.08$ & $\cdots$ & $\cdots$ & $\cdots$ \\
18 & 85.51 & 4.97 & -9.80 & $24.34$ & $0.03$ & $23.80$ & $0.18$ & $-0.54$ & $0.19$ \\
19 & 90.61 & 10.07 & -4.70 & $24.97$ & $0.05$ & $23.45$ & $0.13$ & $-1.52$ & $0.14$ \\
20 & 95.31 & 14.77 & 0.00 & $25.27$ & $0.07$ & $23.41$ & $0.13$ & $-1.85$ & $0.15$ \\
21 & 100.50 & 19.97 & 5.17 & $25.62$ & $0.09$ & $23.47$ & $0.13$ & $-2.15$ & $0.16$ \\
22 & 105.23 & 24.69 & 9.92 & $26.23$ & $0.15$ & $23.95$ & $0.20$ & $-2.28$ & $0.25$ \\
23 & 110.54 & 30.00 & 15.23 & $26.99$ & $0.25$ & $24.01$ & $0.20$ & $-2.98$ & $0.32$ \\
24 & 115.51 & 34.97 & 20.20 & $27.37$ & $0.38$ & $24.28$ & $0.25$ & $-3.09$ & $0.45$ \\
25 & 120.91 & 40.39 & 25.58 & $27.17$ & $0.31$ & $>24.67$ & $\cdots$ & $\cdots$ & $\cdots$ \\
26 & 125.65 & 45.10 & 30.34 & $26.78$ & $0.21$ & $>24.93$ & $\cdots$ & $\cdots$ & $\cdots$ \\
27 & 130.35 & 49.81 & 35.04 & $27.17$ & $0.30$ & $>25.30$ & $\cdots$ & $\cdots$ & $\cdots$ \\
28 & 135.19 & 54.64 & 39.87 & $27.11$ & $0.27$ & $>25.19$ & $\cdots$ & $\cdots$ & $\cdots$ \\
29 & 140.48 & 59.94 & 45.17 & $27.27$ & $0.32$ & $>25.28$ & $\cdots$ & $\cdots$ & $\cdots$ \\
30 & 145.65 & 65.11 & 50.34 & $27.98$ & $0.63$ & $>24.92$ & $\cdots$ & $\cdots$ & $\cdots$ \\
31 & 150.15 & 69.61 & 54.84 & $>27.78$ & $\cdots$ & $>24.99$ & $\cdots$ & $\cdots$ & $\cdots$ \\
32 & 155.45 & 74.91 & 60.14 & $>27.81$ & $\cdots$ & $>25.22$ & $\cdots$ & $\cdots$ & $\cdots$ \\
\hline
\multicolumn{10}{c}{M87 Nova 21} \\
\hline\\
30 & 145.65 & -9.80 & -14.77 & $>26.49$ & $\cdots$ & $>25.11$ & $\cdots$ & $\cdots$ & $\cdots$ \\
31 & 150.15 & -5.30 & -10.27 & $>26.51$ & $\cdots$ & $>25.06$ & $\cdots$ & $\cdots$ & $\cdots$ \\
32 & 155.45 & 0.00 & -4.97 & $23.60$ & $0.04$ & $23.60$ & $0.15$ & $-0.00$ & $0.16$ \\
33 & 160.42 & 4.97 & 0.00 & $24.61$ & $0.10$ & $23.17$ & $0.11$ & $-1.44$ & $0.15$ \\
34 & 165.65 & 10.20 & 5.23 & $25.09$ & $0.15$ & $23.31$ & $0.13$ & $-1.78$ & $0.20$ \\
35 & 170.35 & 14.90 & 9.93 & $25.75$ & $0.26$ & $23.42$ & $0.13$ & $-2.33$ & $0.29$ \\
36 & 175.24 & 19.79 & 14.82 & $26.19$ & $0.42$ & $23.85$ & $0.18$ & $-2.34$ & $0.45$ \\
37 & 180.49 & 25.04 & 20.07 & $26.20$ & $0.40$ & $24.11$ & $0.26$ & $-2.09$ & $0.47$ \\
38 & 185.39 & 29.94 & 24.97 & $26.23$ & $0.41$ & $>24.43$ & $\cdots$ & $\cdots$ & $\cdots$ \\
39 & 190.36 & 34.90 & 29.94 & $>26.52$ & $\cdots$ & $>24.84$ & $\cdots$ & $\cdots$ & $\cdots$ \\
40 & 195.12 & 39.67 & 34.71 & $26.20$ & $0.40$ & $>25.08$ & $\cdots$ & $\cdots$ & $\cdots$ \\
41 & 200.69 & 45.24 & 40.27 & $26.62$ & $0.64$ & $>24.91$ & $\cdots$ & $\cdots$ & $\cdots$ \\
42 & 205.46 & 50.00 & 45.04 & $>26.54$ & $\cdots$ & $>25.02$ & $\cdots$ & $\cdots$ & $\cdots$ \\
43 & 210.49 & 55.04 & 50.07 & $>26.54$ & $\cdots$ & $>24.74$ & $\cdots$ & $\cdots$ & $\cdots$ \\
44 & 215.26 & 59.80 & 54.84 & $26.17$ & $0.40$ & $>25.02$ & $\cdots$ & $\cdots$ & $\cdots$ \\
45 & 220.48 & 65.03 & 60.06 & $>26.20$ & $\cdots$ & $>25.12$ & $\cdots$ & $\cdots$ & $\cdots$ \\
46 & 225.58 & 70.13 & 65.16 & $>26.49$ & $\cdots$ & $>25.08$ & $\cdots$ & $\cdots$ & $\cdots$ \\
\hline
\multicolumn{10}{c}{M87 Nova 22} \\
\hline\\
9 & 40.01 & -15.17 & -10.00 & $>26.78$ & $\cdots$ & $>25.03$ & $\cdots$ & $\cdots$ & $\cdots$ \\
10 & 45.04 & -10.13 & -4.97 & $>26.31$ & $\cdots$ & $>25.07$ & $\cdots$ & $\cdots$ & $\cdots$ \\
11 & 50.01 & -5.17 & 0.00 & $24.57$ & $0.05$ & $22.65$ & $0.08$ & $-1.92$ & $0.10$ \\
12 & 55.17 & 0.00 & 5.17 & $23.64$ & $0.03$ & $23.45$ & $0.14$ & $-0.19$ & $0.14$ \\
13 & 60.07 & 4.90 & 10.07 & $24.33$ & $0.05$ & $22.96$ & $0.09$ & $-1.37$ & $0.10$ \\
14 & 65.13 & 9.97 & 15.10 & $25.16$ & $0.10$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ \\
15 & 70.05 & 14.90 & 20.02 & $25.33$ & $0.11$ & $23.26$ & $0.12$ & $-2.07$ & $0.16$ \\
16 & 75.58 & 20.40 & 25.57 & $25.75$ & $0.17$ & $24.08$ & $0.22$ & $-1.67$ & $0.28$ \\
17 & 80.54 & 25.37 & 30.54 & $25.79$ & $0.15$ & $24.40$ & $0.31$ & $-1.39$ & $0.34$ \\
18 & 85.51 & 30.34 & 35.50 & $26.13$ & $0.22$ & $>24.91$ & $\cdots$ & $\cdots$ & $\cdots$ \\
19 & 90.61 & 35.44 & 40.60 & $25.99$ & $0.19$ & $>25.03$ & $\cdots$ & $\cdots$ & $\cdots$ \\
20 & 95.31 & 40.14 & 45.30 & $26.29$ & $0.25$ & $>24.59$ & $\cdots$ & $\cdots$ & $\cdots$ \\
21 & 100.50 & 45.34 & 50.47 & $26.35$ & $0.28$ & $>25.03$ & $\cdots$ & $\cdots$ & $\cdots$ \\
22 & 105.23 & 50.06 & 55.22 & $26.38$ & $0.27$ & $>24.90$ & $\cdots$ & $\cdots$ & $\cdots$ \\
23 & 110.54 & 55.37 & 60.54 & $26.13$ & $0.22$ & $>24.98$ & $\cdots$ & $\cdots$ & $\cdots$ \\
24 & 115.51 & 60.34 & 65.50 & $26.73$ & $0.39$ & $>25.16$ & $\cdots$ & $\cdots$ & $\cdots$ \\
25 & 120.91 & 65.76 & 70.88 & $27.06$ & $0.51$ & $>24.60$ & $\cdots$ & $\cdots$ & $\cdots$ \\
26 & 125.65 & 70.47 & 75.64 & $>27.13$ & $\cdots$ & $>25.14$ & $\cdots$ & $\cdots$ & $\cdots$ \\
27 & 130.35 & 75.18 & 80.34 & $>26.51$ & $\cdots$ & $>25.10$ & $\cdots$ & $\cdots$ & $\cdots$ \\
\hline
\multicolumn{10}{c}{M87 Nova 23} \\
\hline\\
16 & 75.58 & -15.03 & -24.91 & $>27.06$ & $\cdots$ & $>25.22$ & $\cdots$ & $\cdots$ & $\cdots$ \\
17 & 80.54 & -10.07 & -19.94 & $>27.19$ & $\cdots$ & $>25.22$ & $\cdots$ & $\cdots$ & $\cdots$ \\
18 & 85.51 & -5.10 & -14.97 & $26.86$ & $0.42$ & $>24.31$ & $\cdots$ & $\cdots$ & $\cdots$ \\
19 & 90.61 & 0.00 & -9.87 & $23.66$ & $0.03$ & $23.64$ & $0.14$ & $-0.03$ & $0.14$ \\
20 & 95.31 & 4.70 & -5.17 & $24.73$ & $0.06$ & $23.17$ & $0.10$ & $-1.56$ & $0.12$ \\
21 & 100.50 & 9.91 & 0.00 & $25.43$ & $0.11$ & $22.55$ & $0.07$ & $-2.88$ & $0.13$ \\
22 & 105.23 & 14.62 & 4.75 & $25.58$ & $0.13$ & $23.01$ & $0.10$ & $-2.57$ & $0.16$ \\
23 & 110.54 & 19.93 & 10.06 & $26.05$ & $0.20$ & $23.23$ & $0.11$ & $-2.82$ & $0.23$ \\
24 & 115.51 & 24.90 & 15.03 & $26.73$ & $0.35$ & $23.64$ & $0.15$ & $-3.08$ & $0.39$ \\
25 & 120.91 & 30.33 & 20.41 & $26.49$ & $0.34$ & $24.04$ & $0.22$ & $-2.45$ & $0.41$ \\
26 & 125.65 & 35.04 & 25.17 & $>27.04$ & $\cdots$ & $23.97$ & $0.23$ & $\cdots$ & $\cdots$ \\
27 & 130.35 & 39.74 & 29.87 & $>27.12$ & $\cdots$ & $24.21$ & $0.27$ & $\cdots$ & $\cdots$ \\
28 & 135.19 & 44.58 & 34.70 & $>27.18$ & $\cdots$ & $24.69$ & $0.41$ & $\cdots$ & $\cdots$ \\
29 & 140.48 & 49.87 & 40.00 & $>27.11$ & $\cdots$ & $>24.95$ & $\cdots$ & $\cdots$ & $\cdots$ \\
30 & 145.65 & 55.04 & 45.17 & $>26.16$ & $\cdots$ & $>24.48$ & $\cdots$ & $\cdots$ & $\cdots$ \\
\enddata
\end{deluxetable}\manlabel{tab:big_phot}{3}
